SUCEA: Reasoning-Intensive Retrieval for Adversarial Fact-checking through Claim Decomposition and Editing

Automatic fact-checking has recently received more attention as a means of combating misinformation. Despite significant advancements, fact-checking systems based on retrieval-augmented language models still struggle to tackle adversarial claims, which are intentionally designed by humans to challenge fact-checking systems. To address these challenges, we propose a training-free method designed to rephrase the original claim, making it easier to locate supporting evidence. Our modular framework, SUCEA, decomposes the task into three steps: 1) Claim Segmentation and Decontextualization that segments adversarial claims into independent sub-claims; 2) Iterative Evidence Retrieval and Claim Editing that iteratively retrieves evidence and edits the subclaim based on the retrieved evidence; 3) Evidence Aggregation and Label Prediction that aggregates all retrieved evidence and predicts the entailment label. Experiments on two challenging fact-checking datasets demonstrate that our framework significantly improves on both retrieval and entailment label accuracy, outperforming four strong claim-decomposition-based baselines.

==> main/ethics.tex <==
\section{Ethical Consideration}

==> tables/full_retrieve_result.tex <==
\begin{table*}[!t]
\centering
\resizebox{\textwidth}{!}{%
\addtolength{\tabcolsep}{0.1em}
\begin{tabular}{lcccccccccccccc}
\toprule
 \multirow{4}{*}{Backbone LLM}  & \multicolumn{4}{c}{Top@3} & \multicolumn{4}{c}{Top@5} & \multicolumn{4}{c}{Top@10} \\
        \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
         & \multicolumn{2}{c}{Contriever} & \multicolumn{2}{c}{TFIDF} & \multicolumn{2}{c}{Contriever} & \multicolumn{2}{c}{TFIDF} & \multicolumn{2}{c}{Contriever} & \multicolumn{2}{c}{TFIDF} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13}
        & RAcc. & Recall & RAcc. & Recall & RAcc. & Recall & RAcc. & Recall & RAcc. & Recall & RAcc. & Recall \\
\midrule

\textbf{\fm} \\\noalign{\vskip 0.5ex}



{\base} & 28.5 & 24.8 & 11.0 & 8.9 & 36.0 & 31.0 & 15.5 & 12.8 & 47.5 & 42.6 & 23.5 & 19.0\\
% \hdashline

Llama-3.1 70B & 40.5 & 35.7 & 27.5 & 23.3 & 47.5 & 40.7 & 29.5 & 26.4 & 51.0 & 46.5 & 34.5 & 29.5 \\
GPT-4o mini & 39.5 & 34.9 & 20.5 & 17.4 & 46.5 & 41.1 & 28.5 & 24.0 & 54.0 & 49.2 & 33.5 & 27.9 \\


\hdashline

% \multicolumn{90}{c}{\emph{\textbf{\wice}}} \\\noalign{\vskip 0.5ex}
\textbf{\wice} \\\noalign{\vskip 0.5ex}

{\base}  & 7.0 & 3.0 & 5.3 & 2.5 & 8.7 & 3.8 & 7.0 & 3.3 & 11.7 & 5.0 & 10.9 & 4.3 \\
% \hdashline

Llama-3.1 70B & 11.1 & 4.5 & 7.8 & 3.5 & 14.1 & 5.0 & 9.5 & 4.0 & 16.4 & 6.5 & 14.0 & 5.8 \\
GPT-4o mini & 8.4 & 3.7 & 7.3 & 3.1 & 10.6 & 4.4 & 9.2 & 3.7 & 16.0 & 6.4 & 13.4 & 5.7 \\


\bottomrule
\end{tabular}
}
\caption{ Retrieval evaluation results under \base and \ours
on the \fm and \wice test sets. \textbf{$RAcc.$} and \textbf{$Recall$} separately denote the precision and recall for retrieval evaluation. 
% \hongjun{It is necessary to remove the recall data?}
}
\label{tab:fullretriveresult}
\end{table*}

==> tables/llm_as_ranker_prompt.tex <==
\begin{table}[!t]
\resizebox{\linewidth}{!}{%
\addtolength{\tabcolsep}{-0.1em}
\small
\centering
\begin{tabular}{p{9cm}}
\toprule
\texttt{[FOOLMETWICE]}\\

\textbf{Prompt}\\
...............

\bottomrule
\end{tabular}
}
\caption{vidence Rerank based on Relevance to Claim
Prompt of \ours}
\label{tab:llm_ranker_prompt}
\end{table}
